Chordal Sparsity for Lipschitz Constant Estimation of Deep Neural Networks

Lipschitz constants of neural networks allow for guarantees of robustness in image classification, safety in controller design, and generalizability beyond the training data. As calculating Lipschitz constants is NP-hard, techniques for estimating Lipschitz constants must navigate the trade-off between scalability and accuracy. In this work, we significantly push the scalability frontier of a semidefinite programming technique known as LipSDP while achieving zero accuracy loss. We first show that LipSDP has chordal sparsity, which allows us to derive a chordally sparse formulation that we call Chordal-LipSDP. The key benefit is that the main computational bottleneck of LipSDP, a large semidefinite constraint, is now decomposed into an equivalent collection of smaller ones: allowing Chordal-LipSDP to outperform LipSDP particularly as the network depth grows. Moreover, our formulation uses a tunable sparsity parameter that enables one to gain tighter estimates without incurring a significant computational cost. We illustrate the scalability of our approach through extensive numerical experiments.

==> figures/lc-times.tex <==
\begin{figure}[h]
\centering

\includegraphics[width=0.5\textwidth, height=4cm]{images/alex-2.png}

\caption{
    On the network \red{XXX}, the estimated Lipschitz constant vs the runtime for different methods.
}
\label{fig:lc-times}
\end{figure}



==> sections/admm.tex <==
\section{ADMM}
\label{sec:admm}

\subsection{Vectorized Forms}

Let \(\mrm{vec} : \mbb{R}^{n \times n} \to \mbb{R}^{n^2}\) take a square matrix to vectorized stack of its columns, and similarly define its inverse \(\mrm{mat} : \mbb{R}^{n^2} \to \mbb{R}^{n \times n}\) to map a stack of columns back into a square matrix.
By convention, we will use capital letters for matrices and lower-case letters for their corresponding vectorized forms.
For instance, we write \(x = \mrm{vec}(X)\) and \(X = \mrm{mat}(x)\).
For each clique \(\mcal{C}_k\) define the matrix \(H_k \coloneqq E_{\mcal{C}_k} \otimes E_{\mcal{C}_k}\) via the Kronecker product in order to satisfy the following properties,
\begin{align*}
    x_k = \mrm{vec}(E_{\mcal{C}_k} X E_{\mcal{C}_k} ^\top) = H_k x,
    \quad
    H_k ^\top x_k = \mrm{vec} (E_{\mcal{C}_k}^\top X_k E_{\mcal{C}_k}).
\end{align*}
Also define vectorized sets of semidefinite matrices and the indicator function as
\begin{align*}
    \mcal{S}_k &=
    \braces{v \in \mbb{R}^{\lvert \mcal{C}_k \rvert} : \mrm{mat}(v) \in \mbb{S}_{-} ^{\lvert \mcal{C}_k \rvert}}, \\
    \delta_{\mcal{A}} (x) &=
        \begin{dcases}
            0, &\enskip x \in \mcal{A} \\
            +\infty, &\enskip \text{otherwise}
        \end{dcases}
\end{align*}
Vectorizations of affine matrix-valued functions also have a convenient form.
For instance, \(\mrm{vec}(Z(\gamma))\) is expressed as
\begin{align*}
    z (\gamma)
    = \mrm{vec}(Z_{\mrm{aff}}) + \sum_{i = 1}^{d} \gamma_i \mrm{vec}(Z_{i})
    = z_{\mrm{aff}} + J \gamma,
\end{align*}
with the columns of \(J\) are given by \(\mrm{vec}(Z_{i})\).



\subsection{Augmented Lagrangian}
Introduce the slack variables \(\omega, v_1, \ldots, v_p\), and reformulate~\eqref{eq:p2} as follows,
\begin{align}
\label{eq:p3-base}
\begin{split}
    \underset{\omega, v, \gamma, z}{\text{minimize}}
        &\quad e_{d}^\top \omega + \delta_{\mcal{A}} (\omega, v, \gamma, z) \\
    \text{subject to}
        &\quad \gamma = \omega \\
        &\quad z_k = v_k, \quad k = 1, \ldots, p
\end{split}
\end{align}
were we group \(v = (v_1, \ldots, v_p)\) and \(z = (z_1, \ldots, z_p)\), and also define
{\small
\begin{align*}
    \delta_{\mcal{A}} (\omega, v, \gamma, z)
        = \delta_{\mbb{R}_+} (\gamma)
        + \sum_{k = 1}^{p} \delta_{\mcal{S}_k} (z_k)
        + \delta_0 \parens{z(\omega) - \sum_{k = 1}^{p} H_k ^\top v_k}
\end{align*}
}
Introducing the multipliers \(\lambda = (\lambda_1, \ldots, \lambda_p)\) and \(\mu\), the scaled augmented Lagrangian for~\eqref{eq:p3-base} is as follows,
\begin{align}
\label{eq:p3-lag}
\begin{split}
    &L_\rho (\omega, v, \gamma, z, \mu, \lambda) \\
    &\quad= e_{d}^\top \omega
        + \delta_{\mcal{A}} (\omega, v, \gamma, z)
        + \frac{\rho}{2} \norm{\gamma - \omega + \rho^{-1} \mu}^2
        \\
    &\qquad+ \frac{\rho}{2} \sum_{k = 1}^{p} \norm{z_k - v_k + \rho^{-1} \lambda_k}^2
\end{split}
\end{align}
The ADMM update steps are then
\begin{align}
\label{eq:admm-updates}
\begin{split}
    \omega^{(t+1)}, v^{(t+1)}
        &= \underset{\gamma, v}{\mrm{update}} \enskip L_{\rho} (\omega, v, \gamma^{(t)}, z^{(t)}, \mu^{(t)}, \lambda^{(t)}) \\
    \gamma^{(t+1)}, z^{(t+1)}
        &= \underset{z}{\mrm{update}} \enskip L_{\rho} (\omega^{(t+1)}, v^{(t+1)}, \gamma, z, \mu^{(t)}, \lambda^{(t)}) \\
    \mu^{(t+1)} &= \mu^{(t)} + \rho \parens{\gamma^{(t+1)} - \omega^{(t+1)}} \\
    \lambda_k ^{(t+1)}
        &= \lambda_k ^{(t)} + \rho \parens{z_k ^{(t+1)} - v_k ^{(t+1)}}, \quad k = 1, \ldots, p
\end{split}
\end{align}


